Online Modified Greedy Algorithm for Storage Control under Uncertainty

This paper studies the general problem of operating energy storage under uncertainty. Two fundamental sources of uncertainty are considered, namely the uncertainty in the unexpected fluctuation of the net demand process and the uncertainty in the locational marginal prices. We propose a very simple algorithm termed Online Modified Greedy (OMG) algorithm for this problem. A stylized analysis for the algorithm is performed, which shows that comparing to the optimal cost of the corresponding stochastic control problem, the sub-optimality of OMG is bounded and approaches zero in various scenarios. This suggests that, albeit simple, OMG is guaranteed to have good performance in some cases; and in other cases, OMG together with the sub-optimality bound can be used to provide a lower bound for the optimal cost. Such a lower bound can be valuable in evaluating other heuristic algorithms. For the latter cases, a semidefinite program is derived to minimize the sub-optimality bound of OMG. Numerical experiments are conducted to verify our theoretical analysis and to demonstrate the use of the algorithm.

==> singleStorageProof-conf.tex <==
\section{Analysis for Single Bus Systems}\label{sec:proofSingleBus}
To demonstrate the proof ideas without unfolding all technicalities, we prove Theorem~\ref{thm:main} for a single bus system under the following simplifying assumptions.

\begin{assumption}\label{assume:singleBusProof0}
We assume in this section:
\begin{itemize}
\item the imbalance process $\{\d_t: t\ge 1\}$ is independent and identically distributed (i.i.d.) across $t$ and is supported on a compact interval $[\dmin, \dmax]$;
\item for each $\ell = 1, \dots, L$, the process $\{\p(t,\ell): t \ge 1\}$ is i.i.d. across $t$ and is supported on a compact interval $[\pmin(\ell), \pmax(\ell)]$.
\end{itemize}
\end{assumption}



\begin{assumption}\label{assume:singleBusProof1}
We assume in this section: with probability $1-\epsilon$
\begin{itemize}
\item the imbalance process $\{\d_t: t\ge 1\}$ is independent and identically distributed (i.i.d.) across $t$ and is supported on a compact interval $[\widehat\dmin, \widehat\dmax]$;
\item for each $\ell = 1, \dots, L$, the process $\{\p(t,\ell): t \ge 1\}$ is i.i.d. across $t$ and is supported on a compact interval $[\widehat\pmin(\ell), \widehat\pmax(\ell)]$.
\end{itemize}
\end{assumption}
%The proof for the general case of Theorem~\ref{thm:main} is given in the appendix, where it is decomposed into various extensions of the basic case discussed in this section.
In the rest of this section, we give conditions for parameters $\ks$ and $\W$ such that solving optimization problem \eqref{prob:P3_alg} online will result in a feasible $\{\b_t: t\ge 1 \}$ sequence (Section~\ref{sec:1busFeasible}), characterize the sub-optimality with respect to the sequence of optimal solution of \eqref{prob:P3_alg}, \ie, $\{\un_t,t\geq 1\}$ as a function of $\ks$ and $\W$ and state the semidefinite program for identifying the optimal $\ks$ and $\W$ pair (Section~\ref{sec:1busPerformance}).

\subsection{Feasibility}\label{sec:1busFeasible}
We start with a structural result for the online optimization problem in \eqref{prob:P3_alg}. It follows from Lemma~\ref{lem:ana_sol} which is proved for general cost functions in Appendix~\ref{appendix:convexCost}.
%As a consequence of the analytical solution lemma (Lemma~\ref{lem:ana_sol}) derived for the general convex costs, the following results hold regarding the solution of \Pk{3} at each time period $t$.
\begin{lemma}\label{coro:tech_res}
At each time period $t$, the solution generated by Algorithm~\ref{alg}, $\ie,\,\un_t$, satisfies
\begin{enumerate}
\item $\un_t = \umin$ whenever $\la \bs_t \ge - \W \Dl\g $,
\item $\un_t = \umax$ whenever $\la \bs_t \le - \W \Du\g $,
\end{enumerate}
where
\[
\Dl\g \defeq \inf\left\{\xi \in \partial_{\u_t} \g_t\middle|
\begin{array}{l}
 \u_t\in [\umin,\umax],\,\, \\
\p(t, \ell)\in [\pmin(\ell), \pmax(\ell)],\, \forall \ell,\\
\d_t\in [\dmin, \dmax],\\
\fn_t\in\F, \,\, t \ge 1
\end{array}
\right\},
\]
and
\[
\Du\g \defeq \sup\left\{\xi \in \partial_{\u_t} \g_t\middle|
\begin{array}{l}
 \u_t\in [\umin,\umax],\,\, \\
\p(t, \ell)\in [\pmin(\ell), \pmax(\ell)],\, \forall \ell,\\
\d_t\in [\dmin, \dmax],\\
\fn_t\in\F, \,\, t \ge 1
\end{array}
\right\}
\]
%    $\Dl\g \defeq \inf\{\xi \in \partial_{\u_t} \g_t: \u_t\in [\umin,\umax],\,\,
%    \p(t, \ell)\in [\pmin(\ell), \pmax(\ell)],\, \ell = 1, \dots, L, \,\,
%    \d_t\in [\dmin, \dmax]\}$ and
%    $\Du\g \defeq \sup\{\xi \in \partial_{\u_t} \g_t: \u_t\in [\umin,\umax],\,\,
%    \p(t, \ell)\in [\pmin(\ell), \pmax(\ell)],\, \ell = 1, \dots, L, \,\,
%    \d_t\in [\dmin, \dmax]\}$
 are the greatest lower bound and the least upper bound of the sub-derivatives of $\g_t$,
 %\footnote{Discussions on sub-derivatives of a general, extended real-valued function follow from the footnote in Lemma \ref{lem:ana_sol}.}
respectively. %where $\d_t$, $\p(t, \ell)$, $\forall \ell$ and $\fn_t$ lies in their bounded supp.
\end{lemma}
\begin{remark}[Evaluation of $\Du\g$, $\Dl\g$] Any finite lower bound and upper bound for the sub-derivative of the cost $\g_t$ can be used as $\Dl \g$ and $\Du \g$, respectively. Here we use the greatest lower bound and least upper bound to provide the tightest performance bounds. For cases with simple cost functions, \eg, for idealized storage with $L = 1$, $\Dl \g$ and $\Du \g$ can be easily obtained from $\pmin (\ell)$,  $\pmax(\ell)$, and constants in the cost function $\g_t$ (such as $\alC(\ell)$ and $\alD(\ell)$). In cases where $\g_t$ is differentiable with respect to $\u_t$, $\Du \g$ and $\Dl \g$ may be obtained by solving a simple optimization problem.
\end{remark}
This allows us to construct the following sufficient condition that will assure the feasibility of the $\{\b_t: t\ge 1\}$ sequence induced by the sequence of storage operation generated by Algorithm~\ref{alg}, \ie, $\{\un_t,t\geq 1\}$.
\begin{theorem}[Feasibility]\label{thm:feas_single}
Suppose the initial storage level satisfies $\b(1) \in [\bmin, \bmax]$, then the storage level sequence $\{\b_t: t\ge 1 \}$ induced by the sequence $\ie,\,\{\un_t,t\geq 1\}$ is feasible with respect to storage level constraints, \ie, $\b_t \in [\bmin, \bmax]$ for all $t$, provided that
\begin{align}
\ksmin\le & \ks \le \ksmax, \label{eq:ksbounds}\\
0 < & \W  \le \Wmax, \label{eq:Wbounds}
\end{align}
where
\begin{equation}\label{eq:ineq_1}
\!\!\ksmin\! = \frac{1}{\la} \left[\!-\W \Dl \g + \pos{\umax \!\!- (1-\la)\bmax}\right]\! -\! \bmax,\!\!\!\!\!\!
\end{equation}
\begin{equation}\label{eq:ineq_2}
\!\!\ksmax\! = \frac{1}{\la} \left[\!-\W \Du \g - \pos{(1-\la)\bmin \!\!- \umin}\right]\!- \!\bmin, \!\!\!\!\!\!
\end{equation}
and
\begin{align}\label{eq:W_max}
\!\!\Wmax\!\! =\! \frac{1}{\Du \g\! - \Dl \g} \Big[&\la (\bmax\! - \bmin)\! -\! \pos{(1-\la)\bmin\! -\! \umin}\nn\\
& \quad- \pos{\umax - (1-\la) \bmax}\Big].
\end{align}
\end{theorem}
\begin{IEEEproof}
The result is proved by induction, where Lemma~\ref{coro:tech_res} is used to partially characterize the sequence of storage operation $\{\un_t,\,\t\geq 1\}$.
See Appendix~\ref{sec:app:1bus} for more details.
\end{IEEEproof}



\subsection{Performance}\label{sec:1busPerformance}
In the previous result, we have established that the sequence of storage operation $\{\un_t,t\geq 1\}$ is feasible for the original stochastic optimal control in \eqref{prob:singleBusGeneral} as long as parameters $\ks$ and $\W$ satisfy \eqref{eq:ksbounds} and \eqref{eq:Wbounds}. In the next theorem, we characterize the sub-optimality of $\{\un_t,t\geq 1\}$ for fixed $\ks$ and $\W$.
%Recall that the control action $\uhat_t$ was generated by solving \textbf{P3} satisfies the box constraint: $\uhat_t\in[\umin,\umax]$. Also, Theorem \ref{thm:feas} ensures that by choosing the control parameter $W$ such that $W\in[0,W^{\text{max}}]$, the constraint $\bmin \leq \b_t\leq \bmax$ is satisfied. In other words, by specifying $\ks$ and $\W$ such that $\ks\in[\ksmin,\ksmax]$ and $\W\in[0,\Wmax]$,  the control action solved from the online algorithm \textbf{P3} is a feasible solution to \textbf{P1}. Next, we will provide a performance analysis for the sub-optimal solution for the Lyaunov optimization based online algorithm.
%\onecolumn
\begin{theorem} [Performance]\label{thm:perf_lyap}
The sub-optimality of storage operation $\{\un_t,t\geq 1\}$ is bounded by $\M(\ks)/\W$, that is
\begin{equation}\label{eq:1busiidperf_bdd}
J^\star \le  J(\un) \le J^\star + \M(\ks)/\W,
\end{equation}
%Let $\uhat_t$ be the control action chosen by solving \textbf{P3} and
%\[
%\begin{split}
%\Jk{3}^\star_t=&\sum_{\ell = 1}^L \p(t, \ell) \Bigg(\alI(\ell) \d_t - \alC(\ell)\hC\left( \pos{\uhat_t}\right) \\
%&\quad + \alD(\ell) \hD\left(\neg{\uhat_t}\right) + \alConst(\ell)\Bigg)^+.
%\end{split}
%\]
%Then
% \begin{equation} \label{eq:perf_bdd}
%  \lim_{T \to \infty} \frac{1}{T}\expec \left[ \sum_{t=1}^{T} \Jk{3}^\star_t\right]  \leq \Jk{1}^\star + \frac{\M(\ks) }{\W}.
%\end{equation}
where
\begin{align*}
&\M(\ks)=\Mone(\ks)+\la(1-\la)\Mtwo(\ks),\\
&\Mone(\ks) =\! \frac{1}{2}\! \max\left(\! \left(\umin\!+(1-\la)\ks\right)^2\!\!,\left(\umax\!+(1-\la)\ks\right)^2\! \right)\!,\\
&\Mtwo(\ks)= \max\left( \left(\bmin+\ks\right)^2,\left(\bmax+\ks\right)^2 \right).
\end{align*}
\end{theorem}
\begin{IEEEproof}
A quadratic Lyapunov function is constructed. The relation between the Lyapunov drift and the objective function of the online optimization problem in \eqref{prob:P3_alg} is exploited, which in turn relates to the objective function of the average cost stochastic control problem in \eqref{prob:singleBusGeneral}. Appendix~\ref{sec:app:1bus} contains the whole proof.
\end{IEEEproof}

%\twocolumn

The theorem above guarantees that the worst-case cost (among different uncertainty realizations) of our online algorithm is bounded above by $J^\star + \M(\ks)/\W$. The sub-optimality bound $\M(\ks)/\W$ reduces to a much simpler form if $\la = 1$.
\begin{remark}[Sub-Optimality Bound, $\la =1 $]\label{remark:subo:la1}
For a storage with $\la = 1$, we have \[\M \defeq \M(\ks) = (1/2) \max((\umin)^2, (\umax)^2),\] and the online algorithm is no worse than $\M/\W$ sub-optimal.
 In this case, one would optimize the performance by setting
\[
\W=\Wmax = \frac{(\bmax - \bmin)-(\umax-\umin)}{\Du \g\! - \Dl \g},
\]
and the corresponding
interval $[\ksmin,\ksmax]$ turns out to be a singleton, where
\[
\ksmin=\ksmax=-\frac{\Du \g(\bmax-\umax)+\Dl \g(\umin-\bmin)}{\Du \g\! - \Dl \g}.
\]
%\end{remark}
%\begin{remark}[Optimality for Efficient Unbounded Storage]
Let $\bmax - \bmin = \rho (\umax - \umin)$. Suppose $|\umax| = |\umin|$. For efficient storage ($\la = 1$),  the sub-optimality bound is
\[
\frac{\M}{\W}= \frac{(1/2)(\Du \g - \Dl g)(\umax)^2}{(\bmax- \bmin) - (\umax - \umin)} = \frac{\Du \g - \Dl g}{4(\rho - 1)} \umax.
\]
For fixed $\umax$, as storage capacity increases , \ie,  $\rho \to \infty$, the sub-optimality $(\M/\W) \to 0$. If $\umax$ and $\bmax$ increases with their ratio $\rho$ fixed, the bound increases linearly with $\umax$.
\end{remark}



%Based on the above theorem, we have shown that the online control policy, derived from Lyapunov optimization, is $O( \M(\ks)/{\W})-$optimal. First for $\la=1$, it is easy to see that this online control policy is $O(1/\W)-$optimal. In this case, the performance is optimized by choosing $\W=\Wmax$. Next, in the following theorem, we will find the value of $(\ks,\W)$ that optimizes the sub-optimal bound, for the general case with $\la\in(0,1)$, using convex optimization.
The remaining  case $\la \in (0,1)$ requires solving an optimization program to identify the bound-minimizing parameter pair $(\ks, \W)$. In the next result, we state a semidefinite program to find $(\ks^\star, \W^\star)$ that solves the following  parameter optimization program
\begin{subequations}\label{P3:PO}
\begin{align*}
\opttag{PO:}\minimize & \quad \M(\ks)/\W\\
\st & \quad  \ksmin\le \ks \le \ksmax,\,\, 0< \W \le \Wmax.
\end{align*}
\end{subequations}
In the current form, this program appears to be non-convex. The next result reformulates {\bf PO} into a semidefinite program. Note that $\ksmin$ and $\ksmax$ are linear functions of $\W$ as defined in \eqref{eq:ineq_1} and \eqref{eq:ineq_2}.

\begin{lemma}[Semidefinite Reformulation of {\bf PO}]\label{SDP_P3_PO}
Let symmetric positive definite matrices $\Xumin$, $\Xumax$, $\Xbmin$, and $\Xbmax$ be defined as follows
%\begin{equation}
%\Xumin\!\! = \begin{bmatrix}
%\None&\!\!\umin+(1-\la)\ks\\
%*& 2\W
%\end{bmatrix},
%\Xumax\!\! = \begin{bmatrix}
%\None&\!\!\umax+(1-\la)\ks\\
%*& 2\W
%\end{bmatrix},
%\end{equation}
%\begin{equation}
%\Xbmin\!\! = \begin{bmatrix}
%\Ntwo&\!\!\bmin+\ks\\
%*& \W
%\end{bmatrix},
%\Xbmax\!\! = \begin{bmatrix}
%\Ntwo&\!\!\bmax+\ks\\
%*& \W
%\end{bmatrix},
%\end{equation}
\begin{equation*}
\!\!\Xudot\!\! = \!\!\begin{bmatrix}
\None&\!\!\udot+(1-\la)\ks\\
*& 2\W
\end{bmatrix}, \,\,
\Xbdot\!\! = \!\!\begin{bmatrix}
\Ntwo&\!\!\bdot+\ks\\
*& \W
\end{bmatrix},\!\!
\end{equation*}
where $(\cdot)$ can be either $\max$ or $\min$, and $\None$ and $\Ntwo$ are auxilliary variables. Then {\bf PO} can be solved via the following semidefinite program
\begin{subequations}\label{prob:sdp}
\begin{align}
\!\!\emph{\minimize} \quad & \None+\la(1-\la)\Ntwo \!\!\\
\!\!\emph{\st} \quad & \ksmin\le  \ks \le \ksmax,\,\, 0 <  \W  \le \Wmax, \!\!\\
& \Xumin,\Xumax, \Xbmin, \Xbmax \succeq 0. \!\!
\end{align}
\end{subequations}
\end{lemma}
\begin{IEEEproof}
The result follows from Schur complement. See Appendix~\ref{sec:app:1bus} for details.
\end{IEEEproof}

We close this section by discussing several implications of the performance theorem.
\begin{remark}[Optimality at the Fast-Acting Limit]
Let the length of each time period be $\Delta t$.
At the limit $\Delta t \to 0$, the online algorithm is optimal. Indeed, as discussed in Section~\ref{sec:problem}, both $|\umin|$ and $|\umax|$ are linear in $\Delta t$, such that $|\umax| \to 0$ and $|\umin|\to 0 $ as $\Delta t\to 0$. Meanwhile, $\la \to 1$ as $\Delta t \to 0$. So by Remark~\ref{remark:subo:la1}, it is easy to verify that the sub-optimality $\M/\W$ converges to zero as $\Delta t \to 0$.
\end{remark}

\begin{remark}[Operational Value of Storage and Percentage Cost Savings]\label{remark:vos}
Operational Value of Storage (VoS) is broadly defined as the savings in the long term system cost due to storage operation. Such an index is usually calculated by assuming storage is operated optimally. In stochastic environments, the optimal system cost with storage operation is hard to obtain in general settings. In our notations, let $\u^\mathrm{NS}$ denote the sequence $\{\u_t: \u_t = 0,  t\ge 1 \}$ which corresponds to no storage operation. Then
\[
\mathrm{VoS} = J(\u^\mathrm{NS}) - J^\star,
\]
and it can be estimated by the interval
\[
\left[J(\u^\mathrm{NS})\! -\! J(\u^\star(\Pk{3})),\,\,  J(\u^\mathrm{NS})\! -\! J(\u^\star(\Pk{3})) \!+ \!\frac{\M}{\W} \right].
\]
Additionally, for a storage operation sequence $\u$, the percentage cost savings due to storage can then be defined by $(J(\u^\mathrm{NS}) - J(\u))/J(\u^\mathrm{NS})$. An upper bound of this for any storage control policy can be obtained via $(J(\u^\mathrm{NS}) - J(\u^\star(\Pk{3})) + \M/\W)/J(\u^\mathrm{NS})$, which to an extent summarizes the limit of a storage system in providing cost reduction.
\end{remark}

